Towards Long-Context Time Series Foundation Models

Time series foundation models have shown impressive performance on a variety of tasks, across a wide range of domains, even in zero-shot settings. However, most of these models are designed to handle short univariate time series as an input. This limits their practical use, especially in domains such as healthcare with copious amounts of long and multivariate data with strong temporal and intra-variate dependencies. Our study bridges this gap by cataloging and systematically comparing various context expansion techniques from both language and time series domains, and introducing a novel compressive memory mechanism to allow encoder-only TSFMs to effectively model intra-variate dependencies. We demonstrate the benefits of our approach by imbuing MOMENT, a recent family of multi-task time series foundation models, with the multivariate context.

==> tables/table_pretrained_imputation.tex <==
\begin{table}[h!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{r|cc|cc|cc|cc|cc|cc|cc}
\toprule
\textbf{Model name} & \multicolumn{2}{c}{\texttt{Exchange}} & \multicolumn{2}{c}{\texttt{ETTh1}} & \multicolumn{2}{c}{\texttt{ETTh2}} & \multicolumn{2}{c}{\texttt{ETTm1}} & \multicolumn{2}{c}{\texttt{ETTm2}} & 
\multicolumn{2}{c}{\texttt{Illness}} & \multicolumn{2}{c}
{\texttt{Weather}} \\
& MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE \\
\midrule
Infini-Channel Mixer TM & \textbf{0.149} & \textbf{0.045} & \textbf{0.496} & 0.586 & \textbf{0.291} & \textbf{0.184} & 0.254 & 0.182 & 0.156 & 0.069 & \textbf{0.935} & \textbf{1.807} & 0.082 & 0.066 \\
Univariate TM & 0.185 & 0.070 & 0.500 & \textbf{0.571} & 0.311 & 0.210 & \textbf{0.229} & \textbf{0.136} & \textbf{0.149} & \textbf{0.062} & 1.232 & 2.809 & \textbf{0.079} & \textbf{0.060} \\
\bottomrule
\end{tabular}
}
\caption{Pretrained Imputation Results}
\label{table:pretrained_imputation}
\end{table}


==> tables/table_pretrained_subset.tex <==
\begin{table}[h!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{r|ccccccc}
\toprule

 \textbf{Model} &              \texttt{Exchange} &           \texttt{ETTh1} &           \texttt{ETTh2} &           \texttt{ETTm1} &           \texttt{ETTm2} &          \texttt{Weather} \\ \midrule
Univariate &           0.250 &           0.437 &           0.343 &           0.333 &           0.230 &           0.222 \\ \midrule
Multivariate Infini-Channel Mixer &  \textbf{0.247} &  \textbf{0.436} &  \textbf{0.337} &  \textbf{0.330} &  \textbf{0.228} &  \textbf{0.214} \\
\bottomrule
\end{tabular}
}
\vspace{0pt}
\caption{Averaged MSE [96,192,384] forecasting, for Infini-Channel Mixer \texttt{Tiny MOMENT} and \texttt{Tiny MOMENT} pretrained for one epoch on the Time Series Pile. See full table in the appendix (TODO - write about the pretraining settings) }
\label{tab:metrics_forecast_pretrained_subset}
\end{table}
